Complex box bounds for real maps

In this paper we prove complex bounds, also referred to as a priori bounds, for real analytic (and even C3) interval maps. This means that we associate to such a map a complex box mapping (which provides a kind of Markov structure), together with universal geometric bounds on the shape of the domains. Such bounds show that the first return maps to these domains are well-controlled, and consequently form one of the corner stones in many recent results on one-dimensional dynamics: renormalisation theory, rigidity results, density of hyperbolicity, local connectivity.

==> bib.tex <==
\begin{thebibliography}{TTTT}

\bibitem[AKLS]{AKLS} A. Avila, J. Kahn, M. Lyubich and W. Shen. Combinatorial rigidity for unicritical polynomials. Ann. of Math. 170 (2009) 783-797.

\bibitem[ALdM]{ALdM} A. Avila, M. Lyubich, W. de Melo. Regular or stochastic dynamics in real analytic families of unimodal maps. Invent. Math. 154 (2003), 451-550.

\bibitem[BvS]{BvS} H. Bruin and S. van Strien, Monotonicity of entropy for real multimodal maps, Preprint arXiv:0905.3377.
To appear in J. Amer. Math. Soc. 

\bibitem[CvS]{CvS} T. Clark and S. van Strien, Quasisymmetric rigidity in one-dimensional dynamics, manuscript.

\bibitem[dFdM]{dFdM} E. de Faria and W. de Melo. Rigidity for critical circle maps II. J. Amer. Math. Soc. 13, no. 2 (1999)  343-370.

\bibitem[dMvS]{dMvS} W. de Melo and S. van Strien. One Dimensional Dynamics. Springer. 1993.

\bibitem[GS\'S1]{GSS1}J. Graczyk, D. Sands and G. \'Swi\c atek.
La d\'eriv\'ee schwarzienne en dynamique unimodale. (French. English, French summaries) [Schwarzian derivative in unimodal dynamics]
C. R. Acad. Sci. Paris S\'er. I Math. 332 (2001), no. 4, 329Ð332.

\bibitem[GS\'S2]{GSS2} J. Graczyk D. Sands, G. \'Swi\c atek. Decay of Geometry for Unimodal Maps: Negative Schwarzian Case. Ann. of Math. 161 (2005), 613-677.

\bibitem[G\'S]{GS} J. Graczyk and G. \'Swi\c atek. Polynomial-like mappings induced by real polynomials. In \emph{Dynamical systems and applications}, volume 4 or \emph{World Sci. Ser. Appl. Anal.}, pages 315-328. World Sci. Publ., River Edge, NJ, 1995.

\bibitem[KL]{KL} J. Kahn and M. Lyubich. The quasi-additivity law in conformal geometry. Ann. of Math. 169(2) (2009) 61-593.

\bibitem[K]{Kozlovski-Schwarzian}O. Kozlovski. Getting rid of the negative schwarzian derivative condition. Ann. of Math. 152 (2000), 743-762.

\bibitem[KSvS] {KSS}O. Kozlovski, W. Shen and S. van Strien. Rigidity for real polynomials. Ann. of Math. 165 (2007), 749-841.

\bibitem[KSvS2] {KSS2}O. Kozlovski, W. Shen and S. van Strien. Density of hyperbolicity in dimension one. Ann. of Math. 166 (2007), 145-182.

\bibitem[KvS]{KS} O. Kozlovski and S. van Strien. Local connectivity and quasi-conformal rigidity of non-renormalizable polynomials. Proc. Lond. Math. Soc. (3), 99(2):(2009) 275-296.

\bibitem[Le]{Le} G. Levin. Bounds for maps of an interval with one reflecting critical point. I. Fund. Math. 157 (1998),  287Ð298.

\bibitem[LvS1]{LS-lc} G. Levin and S. van Strien. Local connectivity of the Julia set of real polynomials, Ann. of Math. 147 (1998), no. 3, 471-541. 

\bibitem[LvS2]{LS-inflection} G. Levin and S. van Strien. Bounds for maps of an interval with one critical point of inflection type, Invent. Math. 141 (2000), 399-465.

\bibitem[LvS3]{LS-lf} G. Levin and S. van Strien. Total disconnectedness of Julia sets and absense of invariant linefields for real polynomials, G\'eom\'etrie complexe st syst\`emes dynamiques (Orsay, 1995). Ast\'erisque No. 261 (2000), xii, 161-172.

\bibitem[LiS]{Li-Shen}S. Li and W. Shen, An improved real $C^k$ Koebe principle, Ergod. Theory Dyn. Sys. \textbf{30}(5) (2010), 1485-1494.

\bibitem[LY]{LY} M. Lyubich and M. Yampolsky. Dynamics of quadratic polynomials: complex bounds for real maps. Ann. Inst. Fourier (Grenoble), 47(4):1219-1255, 1997.

\bibitem[M]{McMullen-3mflds} C. T. McMullen. Renormalization and 3-Manifolds which Fiber over the Circle. Annals of Mathematical Studies. 142. Princeton University Press, Princeton, NJ. 1996.

\bibitem[QY]{QY} W. Qiu and Y. Yin. Proof of the Branner-Hubbard conjecture on Cantor Julia sets. Science in China Series A: Mathematics, 52 (1), 45-65, 2009.

\bibitem[RvS1]{RvS1} L. Rempe and S. van Strien. Absence of line fields and Ma\~n\'e's theorem for nonrecurrent
   transcendental functions, Trans. Amer. Math. Soc. 363 (1), 203-228, 2011.
   
\bibitem[RvS2]{RvS2} L. Rempe-Gillen and S. van Strien.   Density of hyperbolicity for classes of real transcendental entire functions and circle maps.  Preprint arXiv:0802.0666. To appear in Duke Math. J.  
   
%\bibitem[NvS]{NS} T. Nowicki and S. van Strien. Properties of $C^{2}$ multimodal Collet-Eckmann maps without Schwarzian derivative assumption. Trans. A. M. S. 321 (2), 1990, 793-810.
\bibitem[S1]{Shen2} W. Shen. Local connectivity of the Julia set of real polynomials (after Levin and van Strien). S\=urikaisekikenky\=usho K\=oky\=uroku, (988):153-159, 1997. Complex dynamical systems and related areas (Japanese) (Kyoto, 1996).

\bibitem[S2]{Shen-lf} W. Shen. On the measurable dynamics of real rational functions. Ergodic Theory Dynam. Systems 23 (2003), 957-983.

\bibitem[S3]{Shen} W. Shen. On the metric properties of multimodal interval maps and $C^{2}$ density of Axiom A. Invent. Math. 156 (2004), 310-401.

\bibitem[Sm]{Sm} D. Smania, Complex bounds for multimodal maps: bounded combinatorics. Nonlinearity 14 (2001), no. 5, 1311Ð1330. 
 
\bibitem[vSV]{vSV} S. van Strien and E. Vargas. Real bounds, ergodicity and negative Schwarzian for multimodal maps. J. Amer. Math. Soc. 17, no. 4 (2004), 749-782.

\bibitem[vSV2]{vSV2} S. van Strien and E. Vargas. Erratum to: ``Real bounds, ergodicity and negative Schwarzian for multimodal maps'' [J. Amer. Math. Soc. 17 (2004), no. 4, 749-782 (electronic); mr2083467]. J. Amer. Math. Soc. 20(1)267-268 (electronic), 2007.

\bibitem[Su]{Sullivan} D. Sullivan. Bounds, renormalization conjectures and quadratic differentials, AMS Centennial Publications II, \emph{Mathematics into the Twenty-First Century}, 417-466, 1992.
\end{thebibliography}
